Ghost Echoes: Semantic Erasure Failure in Retrieval-Backed Applications

Although vector databases correctly implement API-visible deletion, this does not guarantee complete semantic erasure for retrieval-backed applications. We present Ghost Echoes, a black-box attack framework showing that deleted records can leave measurable residual influence on downstream retrieval contexts. Our primary finding is the RAG retrieval-context drift effect where even when a target record is correctly excluded from query results, its prior presence perturbs the semantic centroid and textual composition of the Top-K evidence base. We approximate the unobservable never-inserted counterfactual using a same-cluster non-target deletion control that preserves local neighborhood structure while isolating target-specific effects from generic local drift. Evaluation on ChromaDB confirms target deletion produces a median retrieval-centroid drift of 0.1522, exceeding the same-cluster baseline in 53/54 paired comparisons (p < 0.001), and the signal remains detectable with 61.1% accuracy at a query budget of q = 5. We verify API-visible deletion correctness across evaluated backends and observe the same qualitative drift ordering in matched FAISS replication. Under the evaluated settings, tested operational mitigations such as full index rebuilds fail to eliminate the measured drift. These results establish a measurable 'verification gap' between interface-level deletion compliance and true semantic erasure, and motivate erasure primitives that act not only on stored identifiers, but also on the retrieval topology of the system.

==> sections/10_limitations.tex <==
% \section{Limitations}
% \label{sec:limitations}

% We conclude with an honest assessment of the limitations of this work.

% \subsection{Threat Model Scope}
% This paper studies a \textbf{black-box attacker with API-only access}. We do not consider storage-layer adversaries or multi-tenant isolation breaches. The attacker relies only on observable retrieval behavior, not model weights.

% \subsection{Claim Boundaries}
% The observed \textbf{RAG retrieval-context drift} measures semantic perturbation of the evidence base. We do not claim this equates to document-level re-identification or exact vector recovery. This paper evaluates \textbf{retrieval-context drift}—the shift in Top-$K$ retrieved documents—not end-to-end LLM answer-generation drift. Purely passive rank-only signals (Phantom Neighborhood) are \textbf{scale-dependent} ($N \ge 5000$).

% \subsection{Backend Coverage Boundary}
% Direct quantification of the RAG retrieval-context drift and mitigation evaluation is currently verified for \textbf{ChromaDB only}. Cross-backend quantification is future work. We provide cross-backend evidence for API exclusion correctness and the underlying induction mechanism, but direct drift tables are bounded to the evaluated settings.

% \subsection{What Ghost Echoes Does Claim}
% \begin{itemize}
%     \item API-visible deletion semantics are enforced correctly on tested backends.
%     \item Semantic erasure failure remains measurable through black-box API interaction.
%     \item \textbf{RAG retrieval-context drift} occurs upon deletion of Top-$K$ members, shifting the semantic centroid by 0.1522 and the textual vocabulary by 25--32\% in the evaluated setting.
%     \item The observed drift is target-specific and distinguishable from index noise (3.7$\times$ control separation).
%     \item Tested mitigations in the evaluated settings did not eliminate the observed retrieval-context drift.
% \end{itemize}

% \subsection{What Ghost Echoes Does Not Claim}
% \begin{itemize}
%     \item Document-level re-identification or exact vector recovery.
%     \item \textbf{LLM answer-generation drift}.
%     \item \textbf{Universal passive rank-drift} for small indices.
%     \item Storage-layer persistence or universal cross-backend drift magnitude without direct evaluation.
% \end{itemize}

% \subsection{Future Work}
% Future research directions include cross-backend quantification of drift and evaluation of LLM answer-generation drift.

